Measurements of electroweak $Wjj$ production and constraints on anomalous gauge couplings with the ATLAS detector

Measurements of the electroweak production of a $W$ boson in association with two jets at high dijet invariant mass are performed using $\sqrt{s} = 7$ and $8$ TeV proton-proton collision data produced by the Large Hadron Collider, corresponding respectively to 4.7 and 20.2 fb$^{-1}$ of integrated luminosity collected by the ATLAS detector. The measurements are sensitive to the production of a $W$ boson via a triple-gauge-boson vertex and include both the fiducial and differential cross sections of the electroweak process.

==> atlas-diffxsec.tex <==

Differential cross sections for \wjets production are measured with the higher integrated luminosity 
$\sqrt{s}=8$~\TeV~data set as a function of a variety of observables (detailed below) and in a number of 
fiducial phase-space regions.  The combined QCD+EW \wjets production is measured in all regions to test 
the modelling of QCD \wjets production.  In regions sensitive to EW \wjets contributions, the 
prediction for QCD \wjets only is shown along with the combined QCD+EW \wjets prediction in order to 
indicate the effect of the EW \wjets process.  Differential measurements of EW \wjets production are 
performed in regions with $\mjj>1.0$~\TeV.  
 
All differential production cross sections are measured both as absolute cross sections and as distributions 
normalized by the cross section of the measured fiducial region ($\sigma^\mathrm{fid}_W$).  Many sources of uncertainty 
are reduced for normalized distributions, allowing higher-precision tests of the modelling of the shape of the 
measured observables in Monte Carlo simulations.  The reported cross sections include the branching fraction for 
the $W\to\ell^\pm\nu$ decay of a single flavour and are normalized by the width of the measured bin interval.  
This section discusses representative differential measurements, with additional distributions provided in 
Appendix~\ref{sec:appendix}.  The complete set of measurements is available in \textsc{hepdata}\,\cite{HEPDATA}.

The MC simulations are used to correct the cross sections for detector and event selection 
inefficiencies, and for the effect of detector resolutions.  An implementation\,\cite{Adye:2011gm} of a 
Bayesian iterative unfolding technique\,\cite{DAgostini2010} is used to perform these corrections. 
The unfolding is based on a response matrix from the simulated events which encodes bin-to-bin migrations between a 
particle-level differential distribution and the equivalent reconstruction-level distribution.  The matrix gives 
transition probabilities from particle level to reconstruction level, and Bayes' theorem is employed to calculate the 
inverse probabilities.  These probabilities are used in conjunction with a prior particle-level signal distribution, 
which is implicitly taken from the \powheg + \pythia simulations, to unfold the background-subtracted 
reconstruction-level data distributions.  After this first unfolding iteration the unfolded data distribution is used 
as the new prior and the process repeated for another iteration.  The unfolding procedure is validated by unfolding 
the \sherpa simulation using the \powheg + \pythia response matrix.  For all distributions the unfolded and initial 
particle-level \sherpa predictions agree within the unfolding uncertainty assigned. Bin boundaries in unfolded 
distributions are chosen to ensure that $>66\%$ of particle-level events remain within the same interval at 
reconstruction level.

Unfolded differential cross-section measurements are compared to theoretical predictions for QCD+EW~\wjets production 
from the \powheg + \pythia, \sherpa, and \textsc{hej} event generators, which are described in 
Section~\ref{sec:mc}.  The normalizations are performed self-consistently, i.e. data measurements are normalized by 
the total fiducial data cross section and MC predictions are normalized by the corresponding MC cross section.

\subsection{Observables and fiducial regions}
\label{sec:diff:obs}

Differential measurements are performed in distributions that provide discrimination between strong and electroweak 
\wjets production, and enhanced sensitivity to anomalous gauge couplings.  The observables sensitive to electroweak 
\wjets production are:
\begin{itemize}
\item $C_\ell$, lepton centrality, the location in rapidity of the lepton relative to the average rapidity of the 
two highest-\pt jets, defined in Eq.~(\ref{eqn:lepcentrality});
\item $C_j$, jet centrality, the location in rapidity of any additional jet relative to the average rapidity of 
the two highest-\pt jets, defined in Eq.~(\ref{eqn:lepcentrality});
\item $\mjj$, the invariant mass of the two highest-$\pt$ jets;
\item $\dyjj$, the absolute rapidity separation between the two highest-$\pt$ jets; 
\item $\ngapjet$, the number of additional jets in the rapidity gap bounded by the two highest-$\pt$ jets 
(i.e., jets with $C_j < 0.5$).


\end{itemize}
Additional observables sensitive to anomalous couplings are:
\begin{itemize}
\item $\ptjlead$, the $\pt$ of the highest-$\pt$ jet;
\item $\pt^{jj}$, the $\pt$ of the dijet system (vector sum of the $\pt$ of the two highest-\pt jets); 
\item $\Delta \phi(j_1,j_2)$, the magnitude of the azimuthal angle between the two highest-$\pt$ jets,
\end{itemize}
where the last observable is sensitive specifically to CP-violating couplings.

The differential cross sections of the combined \wjets processes are measured in the following nine fiducial regions:
\begin{itemize} 
\item Four mutually orthogonal fiducial regions defined in Figure~\ref{evtsel:phasespaceIllustration}, three of which 
are electroweak-suppressed ($<5\%$ contribution) and one electroweak-enhanced ($15$--$20\%$ contribution);
\item An additional electroweak-enhanced signal region with $\mjj>1.0$~\TeV~($35$--$40\%$ electroweak \wjets 
contribution);
\item Four inclusive fiducial regions defined by the preselection requirements in Table~\ref{tab:selection} 
with $\mjj > 0.5,~1.0,~1.5$~and~2.0~\TeV.
\end{itemize}

The inclusive fiducial regions probe the observables used to separate the signal and control or validation regions, 
namely lepton and jet centrality, as well as the number of jets radiated in the rapidity gap between the two leading 
jets.  The four successively higher invariant mass thresholds increasingly enhance the EW~\wjets purity of the 
differential distributions, without the lepton and jet topology requirements applied to the dedicated signal-enhanced 
regions.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.45\textwidth]{figures/unfolding/EWKfraction/predictedEWKfraction_ngapjets_1D_inclusive.pdf}
\includegraphics[width=0.45\textwidth]{figures/unfolding/EWKfraction/predictedEWKfraction_dijetmass_1D_signal.pdf}
\caption{Fraction of EW~\wjets signal relative to the combined QCD+EW~\wjets production, 
predicted by \powheg + \pythia and \sherpa simulations for observables in the inclusive and signal regions.}
\label{unfolding:EWKfraction}
\end{figure}

Figure~\ref{unfolding:EWKfraction} shows the \powheg + \pythia and \sherpa predictions of the fraction of \wjets 
events produced via electroweak processes, as a function of the number of jets emitted in the dijet rapidity 
gap for the inclusive fiducial regions with $\mjj>0.5$~TeV and the dijet invariant mass in the signal 
fiducial region.
The EW~\wjets signal is enhanced in events with zero jets in 
the dijet rapidity gap due to the absence of colour connection between the incoming partons.  

In addition to the measurements of differential cross sections for combined QCD+EW \wjets production in the 
nine fiducial regions listed above, EW~\wjets differential cross sections are extracted in four fiducial 
regions that have an expected EW~\wjets fraction of $>20\%$: the three highest 
invariant-mass inclusive regions ($\mjj>1.0$~\TeV, 1.5~\TeV, and 2.0~\TeV), and the high-mass signal region 
($\mjj>1.0$~\TeV); the latter has the highest expected total EW~\wjets signal purity, about $40\%$.  The 
QCD \wjets background is subtracted using the multiplicative normalization factor of $\muqcd = 1.09 \pm 0.02$~(stat) 
determined from the fits in Section~\ref{sec:xsec}.  This substantially reduces the normalization uncertainty, 
confining theoretical uncertainties to the shapes of the background distributions.

Performing a complete unfolding of the EW~\wjets signal process leads to better precision on the unfolded 
data, particularly in the case of normalized distributions, than could be achieved by subtracting the 
particle-level QCD~\wjets production background from unfolded QCD+EW~\wjets production data.  
All EW~\wjets differential measurements are nonetheless also performed as combined QCD+EW \wjets production 
measurements so that such a subtraction could be performed with other QCD \wjets predictions.

\subsection{Uncertainties}
\label{sec:diff:syst}

The sources of uncertainty discussed in Section~\ref{sec:xsec} are assessed for the unfolded 
differential production cross sections.  Figures are shown with statistical uncertainties as 
inner bars and total uncertainties as the outer bars.

Statistical uncertainties are estimated using pseudoexperiments, with correlations between bins determined 
using a bootstrap method\,\cite{Hayes:1988xc}.  The $W\to e\nu$ and $W\to\mu\nu$ channels are found to be 
statistically compatible, and are combined.  Theoretical uncertainties include the effects of scale and PDF 
variations on the prior distribution and on the response matrix.  For unfolding EW \wjets production, additional 
theoretical uncertainties arise from modelling the QCD \wjets contribution subtracted from the data, and from 
the neglect of interference between the strong and electroweak \wjets processes.  
The interference uncertainty is estimated using the same procedure as for the fiducial measurement 
(Section~\ref{sec:xsec}), i.e. by adding the \sherpa interference model to the background prediction.  An 
uncertainty in the unfolding procedure is estimated by reweighting the simulation such that the distributions 
match the unfolded data, and then unfolding the data with the reweighted simulation; the change in the unfolded 
measurement is symmetrized and taken as an uncertainty.  Experimental uncertainties are assessed by unfolding 
the data distributions using a modified response matrix and prior incorporating the change in detector response. 

Figure~\ref{unfolding:systSummary_examples} summarizes the statistical uncertainties and the statistical and 
systematic uncertainties summed in quadrature of the unfolded distributions for a selection of observables 
for the combined QCD+EW~\wjets processes.  The jet energy scale and resolution uncertainties dominate 
the total uncertainty except in regions where statistical uncertainties are significant.  The unfolding 
uncertainty is typically relevant in these regions and in regions dominated by QCD \wjets production where 
the statistical uncertainties are small. 

\begin{figure}[!tbp]
\centering
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryAbsXSec_combined_ngapjets_1D_inclusive.pdf}
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryAbsXSec_combined_LC_1D_highmass10.pdf}
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryAbsXSec_combined_dijetmass_1D_inclusive.pdf}
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryAbsXSec_combined_dijetpt_1D_signal.pdf}
\caption{Relative uncertainties in example unfolded differential cross sections for the combined QCD+EW~\wjets 
processes.  The examples are: the number of jets in the rapidity gap between 
the two highest-$\pt$ jets in the inclusive region (top left); the lepton centrality distribution in the inclusive 
$\mjj>1$~TeV region (top right); $\mjj$ in the inclusive region (bottom left); and the dijet $\pt$ in the signal 
region (bottom right). Dominant contributions to the total systematic uncertainty are highlighted separately.}
\label{unfolding:systSummary_examples}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryEWKAbsXSec_combined_dijetmass_1D_signal10.pdf}
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryEWKAbsXSec_combined_dy12_1D_signal10.pdf}
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryEWKAbsXSec_combined_dijetmass_1D_highmass10.pdf}
\includegraphics[width=0.49\textwidth]{figures/unfolding/systSummary/systematicSummaryEWKAbsXSec_combined_j1pt_1D_signal10.pdf}
\caption{Relative uncertainties in example unfolded differential cross sections for the EW \wjets processes.  
The examples are $\mjj$ (top left) and $\dyjj$ (top right) in the high-mass signal region; $\mjj$ in the 
$\mjj>1$~TeV inclusive region (bottom left); and leading-jet $\pt$ in the high-mass signal region (bottom right).
Dominant contributions to the total systematic uncertainty are highlighted separately. }
\label{unfolding:systSummaryEWK_examples}
\end{figure}

Figure~\ref{unfolding:systSummaryEWK_examples} summarizes the uncertainty contributions to example EW \wjets unfolded 
data distributions.  Uncertainties in the modelling of strong \wjets production are particularly important at low 
dijet invariant mass, where the EW~\wjets signal purity is lowest.  Interference uncertainties become 
dominant at low dijet rapidity separation but are otherwise not the leading contribution to the total uncertainty.  
A recent study\,\cite{Denner:2014ina} of interference in $Z$+jets vector-boson-fusion topologies, incorporating 
NLO electroweak corrections, predicted similar behaviour.  
For the bulk of the EW \wjets distributions, the leading sources of uncertainty are statistical, QCD \wjets modelling, 
and jet energy scale and resolution, and contribute roughly equally.

\subsection{Combined strong and electroweak \wjets measurements}

This section reports the combined strong and electroweak \wjets differential cross-section results, with comparisons to 
the MC predictions given by \sherpa, \powheg + \pythia, and \textsc{hej}.  Comparisons to \textsc{hej} are only performed in 
regions of high purity for strong \wjets production, as discussed in Section~\ref{sec:mc}.

Figure~\ref{unfolding:norm_measurementngapjets}~shows the normalized differential cross section as a function of 
the number of $\pt>30$~\GeV~jets emitted into the rapidity gap for progressively increasing \mjj thresholds.  In 
the lowest invariant-mass fiducial region, strong \wjets production dominates and predictions from \powheg + \pythia, 
\sherpa, and \textsc{hej} all describe the data well, for up to eight additional jet emissions. As the dijet invariant 
mass threshold is increased, the differences in shape between predictions with and without the EW~\wjets 
contribution become apparent.

The value in the zero-jet bin corresponds to the efficiency of a central jet veto for each dijet invariant mass 
threshold.  This efficiency is higher for EW~\wjets production due to the absence of colour exchange; 
as the \mjj threshold increases the EW \wjets purity increases and its effect on the efficiency increases.  
Table~\ref{tab:jetvetoeff} summarizes the measured jet-veto efficiency and the predictions from \powheg + \pythia 
QCD and QCD+EW \wjets simulations.  The data efficiencies quoted in Table~\ref{tab:jetvetoeff} show compatibility 
with the efficiencies of the combined \wjets processes in the simulation.

Jet centrality is related to the number of jets in the rapidity gap, as events with $C_j < 0.5$ have a jet within the 
gap.  Figure~\ref{unfolding:combined_measurementLC1Dinclusive} shows good agreement between the predictions and data 
in the differential cross section weighted by the mean number of gap jets.

The differential cross section in the inclusive region as a function of lepton centrality is shown in 
Figure~\ref{unfolding:combined_measurementLC1Dinclusive} for two $\mjj$ thresholds.  These measurements 
indirectly probe the rapidity of the $W$~boson relative to the dijet rapidity interval. Data with lepton 
centrality below 0.4 correspond to the presence of a lepton inside the rapidity region defined in 
Figure~\ref{evtsel:vetoIllustration}.  All theoretical predictions adequately describe the lepton centrality 
in the region with the lowest dijet mass threshold, which is dominated by QCD \wjets production.  As the 
$\mjj$ threshold is increased the differences between QCD and QCD+EW \wjets production become more apparent, 
particularly at low lepton centrality where EW~\wjets production is enhanced.  At even larger invariant 
masses, \sherpa predicts a higher rate than data in the high-centrality, or forward-lepton, region (see 
Appendix~\ref{sec:appendix}). 

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_ngapjets_1D_inclusive}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_ngapjets_1D_highmass10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_ngapjets_1D_highmass15}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_ngapjets_1D_highmass20}
\caption{Unfolded normalized distribution of the number of jets with $\pt>30$~\GeV~in the rapidity interval bounded 
by the two highest-$\pt$ jets in the inclusive fiducial region with $\mjj$ thresholds of 
0.5~\TeV~(top left),~1.0~\TeV~(top right),~1.5~\TeV~(bottom left), and 2.0~\TeV~(bottom right).  Both statistical 
(inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios of the theoretical 
predictions to the data (the bottom panel in each distribution).  }
\label{unfolding:norm_measurementngapjets}
\end{figure}

\begin{table*}[htbp]
\caption{
Jet-veto efficiency for each $\mjj$ threshold compared to \powheg + \pythia QCD+EW and QCD \wjets simulations.  
The uncertainties comprise statistical and systematic components added in quadrature.}
\label{tab:jetvetoeff}
\begin{center}
\begin{tabular}{l|cccc}
\toprule
 & \multicolumn{4}{c}{Jet-veto efficiency} \\
& $\mjj>0.5$~TeV & $\mjj>1.0$~TeV &$\mjj>1.5$~TeV &$\mjj>2.0$~TeV \\
\midrule
Data                       & $0.596\pm 0.014$ & $0.54\pm 0.02$ & $0.55\pm 0.03$ & $0.63\pm 0.04$ \\
\powheg+\pythia (QCD+EW) & $0.597\pm 0.005$ & $0.55\pm 0.01$ & $0.57\pm 0.02$ & $0.63\pm 0.03$ \\
\powheg+\pythia (QCD) & $0.569\pm 0.002$ & $0.45\pm 0.01$ & $0.39\pm 0.01$ & $0.36\pm 0.03$ \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_JC_1D_inclusive}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_JC_1D_highmass10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_LC_1D_inclusive}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_LC_1D_highmass10}
\caption{Unfolded normalized differential \wjets production cross sections as a function of jet centrality (top) 
and lepton centrality (bottom) for the inclusive fiducial region with $\mjj > 0.5$~\TeV~(left) and 1.0~\TeV~(right).  
Both statistical (inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios of 
the theoretical predictions to the data (the bottom panel in each distribution).}
\label{unfolding:combined_measurementLC1Dinclusive}
\end{figure}

\begin{figure}[htbp]\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dijetmass_1D_inclusive}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dijetmass_1D_antiLC}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dijetmass_1D_antiJC}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dijetmass_1D_antiLCantiJC}
\caption{Unfolded differential \wjets production cross sections as a function of dijet mass for the inclusive (top left), 
forward-lepton (top right), central-jet (bottom left), and forward-lepton/central-jet (bottom right) fiducial regions, 
which are enriched in strong \wjets production.  Both statistical (inner bar) and total (outer bar) measurement 
uncertainties are shown, as well as ratios of the theoretical predictions to the data (the bottom panel in each 
distribution).}
\label{unfolding:combined_measurementdijetmass1Dinclusive}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dy12_1D_antiLC}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dy12_1D_antiJC}
\caption{Unfolded absolute differential \wjets production cross sections as a function of dijet rapidity separation 
for the forward-lepton control and central-jet validation regions, which are dominated by strong \wjets production.  
Both statistical (inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios of the 
theoretical predictions to the data (the bottom panel in each distribution).}
\label{unfolding:combined_measurementdy121DantiLC}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dijetmass_1D_signal}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dijetmass_1D_signal}
\caption{Unfolded absolute (left) and normalized (right) differential \wjets production cross section as a function 
of dijet mass for the signal fiducial region.  Both statistical (inner bar) and total (outer bar) measurement 
uncertainties are shown, as well as ratios of the theoretical predictions to the data (the bottom panel in each 
distribution).}
\label{unfolding:combined_measurementdijetmass1Dsignal}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dy12_1D_inclusive}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dy12_1D_highmass10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dy12_1D_highmass15}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_dy12_1D_highmass20}
\caption{Unfolded absolute differential \wjets production cross sections as a function of $\dyjj$ for the inclusive 
fiducial region with progressively increasing dijet mass thresholds.  Both statistical (inner bar) and total 
(outer bar) measurement uncertainties are shown, as well as ratios of the theoretical predictions to the data 
(the bottom panel in each distribution).}
\label{unfolding:combined_measurementdy121Dinclusive}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dy12_1D_signal}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dy12_1D_signal10}
\caption{Unfolded normalized differential \wjets production cross sections as a function of $\dyjj$ for the 
signal regions with $\mjj > 0.5$~\TeV~(left) and $\mjj > 1.0$~\TeV~(right).  Both statistical
(inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios of the theoretical 
predictions to the data (the bottom panel in each distribution). }
\label{unfolding:combined_measurementdy121Dsignal}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dphi12_1D_inclusive}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dphi12_1D_antiLC}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dphi12_1D_antiJC}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dphi12_1D_signal}
\caption{Unfolded normalized differential \wjets production cross sections as a function of $\Delta\phi(j_1,j_2)$ 
for the inclusive, forward-lepton control, central-jet validation, and signal fiducial regions.  Both statistical
(inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios of the theoretical 
predictions to the data (the bottom panel in each distribution). }
\label{unfolding:combined_measurementdphi121Dinclusive}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dijetpt_1D_inclusive}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dijetpt_1D_highmass10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dijetpt_1D_signal}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/measurement_combined_dijetpt_1D_signal10}
\caption{Unfolded normalized differential \wjets production cross sections as a function of dijet $\pt$ for the 
inclusive (top) and signal (bottom) regions with $\mjj>0.5$~\TeV~(left) and $\mjj > 1.0$~\TeV~(right). Both 
statistical (inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios of the 
theoretical predictions to the data (the bottom panel in each distribution).}
\label{unfolding:combined_measurementdijetpt1Dinclusive}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_j1pt_1D_antiLC}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_j1pt_1D_antiLCantiJC}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_j1pt_1D_signal}
\includegraphics[width=0.48\textwidth]{figures/unfolding/absoluteXsec/measurementAbsXSec_combined_j1pt_1D_signal10}
\caption{Unfolded absolute differential \wjets production cross sections as a function of leading-jet $\pt$ for the 
forward-lepton control region, forward-lepton/central-jet fiducial region, and for the signal regions with 
$\mjj>0.5$~TeV and 1.0~\TeV.  Both statistical (inner bar) and total (outer bar) measurement uncertainties are 
shown, as well as ratios of the theoretical predictions to the data (the bottom panel in each distribution). }
\label{unfolding:combined_measurementj1pt1DantiLC}
\end{figure}

Figure~\ref{unfolding:combined_measurementdijetmass1Dinclusive} shows the cross sections as a function 
of the dijet invariant mass in four fiducial regions enriched in strong \wjets production: the inclusive region, the 
forward-lepton control region, the central-jet validation region, and the forward-lepton/central-jet validation region.
Predictions from \textsc{hej}, which are expected to provide a good description of strong \wjets production at high dijet 
invariant mass where large logarithms contribute, are similar to the NLO predictions from \powheg + \pythia. 
\sherpa predicts more events at high dijet invariant mass than observed in data in these fiducial regions, and has a 
larger disagreement in shape with the data, than \powheg + \pythia or \textsc{hej}.
The dijet rapidity separation (Figure~\ref{unfolding:combined_measurementdy121DantiLC}) also discriminates between 
strong (at low separation) and electroweak (at high separation) \wjets production, and is generally well modelled by the 
different predictions in the forward-lepton and central-jet fiducial regions where strong \wjets production 
dominates (although there are some shape differences between data and \textsc{hej} in the forward-lepton 
control region).

In the signal region (Figure~\ref{unfolding:combined_measurementdijetmass1Dsignal}), the discrimination power between 
electroweak and strong \wjets predictions is enhanced, with the data supporting the presence of electroweak \wjets 
production.  The excess of \powheg + \pythia over data at high \mjj is consistent with a measured $\muew < 1$ (see 
Sec.~\ref{sec:fidxsresults}).  

Figure~\ref{unfolding:combined_measurementdy121Dinclusive} shows the dijet rapidity interval distribution in the 
inclusive region with increasing $\mjj$ thresholds that increasingly enhance the EW~\wjets signal.  The 
predictions from all generators broadly describe the data.  The ratio of the \powheg + \pythia strong \wjets 
prediction to the data has a negative slope, predicting smaller interval sizes than observed and demonstrating the 
presence of an EW~\wjets signal component.

The behaviour of the EW~\wjets signal as a function of the dijet rapidity interval distribution is further studied 
in Figure~\ref{unfolding:combined_measurementdy121Dsignal}, which shows a clear difference between the predictions 
with and without the EW~\wjets process.
Both \powheg + \pythia and \sherpa describe the data distribution reasonably well in these signal-enhanced 
regions with $\mjj>0.5$~\TeV~and 1.0~\TeV.  Predictions from \textsc{hej} show shape differences with respect to 
the data at the $\approx 10\%$ level. 

The normalized differential cross sections for \wjets production as a function of the azimuthal angle between the two 
leading jets are shown in the inclusive, forward-lepton control, central-jet validation, and signal fiducial regions in 
Figure~\ref{unfolding:combined_measurementdphi121Dinclusive}.  Good agreement between the data and all predictions is 
seen, with a slight tendency for predictions to overestimate the relative rate at small angles in all fiducial regions.

Figure~\ref{unfolding:combined_measurementdijetpt1Dinclusive} shows the measured normalized \pT distribution of the 
dijet system compared to the various predictions.  There is a trend for all predictions to overestimate the relative 
rate at high dijet $\pt$ in the inclusive and signal-enhanced regions, while the central-jet validation region (shown 
in Appendix~\ref{sec:appendix}) does not show such a trend.  Increasing the dijet invariant mass threshold to enhance 
the EW~\wjets signal does not increase the magnitude of the disagreement with data, suggesting that the 
difference is related to the modelling of the QCD~\wjets production.  Recent studies\,\cite{openloops1} of NLO 
electroweak corrections to strong \wjets production predict negative corrections to the production cross section at 
high $W$-boson and leading-jet $\pt$, offering a possible explanation for this discrepancy.

The transverse momentum distribution of the leading jet, shown in Figure~\ref{unfolding:combined_measurementj1pt1DantiLC}, 
is globally well described by \powheg + \pythia.  Predictions from \sherpa and \textsc{hej} both show a harder spectrum 
than observed in data, with this behaviour seen in regions that are enriched in either QCD~\wjets production or in 
EW~\wjets production.  Comparisons of unfolded data and theoretical predictions in the inclusive fiducial 
regions are shown in Appendix~\ref{sec:appendix} (Figure~\ref{unfolding:combined_measurementj1pt1Dinclusive}).


\subsection{Electroweak \wjets measurements}
\label{sec:diffxsec:ewonly}

As discussed in Section~\ref{sec:diff:obs}, cross sections of pure electroweak \wjets production are measured in 
fiducial regions with high EW \wjets purity.  Additional uncertainties in the modelling of strong \wjets 
production and the interference between the strong and electroweak \wjets processes are included, as discussed in 
Section~\ref{sec:diff:syst}.  
The interference uncertainty is shown explicitly as a shaded area in each bin of the measured distributions.
Results are presented in the EW~\wjets signal region defined in Table~\ref{tab:selection} and the inclusive 
regions with dijet mass requirements of $\mjj>1.0$, 1.5, and 2.0~\TeV.  A subset of the measured differential results 
are shown here; additional distributions are tabulated in \textsc{hepdata}. 
Results are compared to EW \wjets predictions from \sherpa and \powheg + \pythia.

\begin{figure}[tbp]
\centering
\includegraphics[width=0.47\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_ngapjets_1D_highmass10}
\includegraphics[width=0.47\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_ngapjets_1D_highmass20}
\caption{Unfolded normalized differential EW~\wjets production cross sections as a function of the number of 
jets with $\pt>30$~\GeV~in the rapidity interval bounded by the two highest-$\pt$ jets in the inclusive fiducial 
region, with $\mjj> 1.0$~\TeV~(left) and $\mjj > 2.0$~\TeV~(right).  Both statistical (inner bar) and total (outer bar) 
measurement uncertainties are shown, as well as ratios of the theoretical predictions to the data (the bottom panel in 
each distribution). }
\label{unfolding:EWKcombined_measurementngapjets1Dhighmass10_15}
\end{figure}

\begin{figure}[tbp]
\centering
\includegraphics[width=0.47\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dijetmass_1D_highmass10}
\includegraphics[width=0.47\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dijetmass_1D_signal10}
\caption{Unfolded normalized differential EW~\wjets production cross sections as a function of the dijet 
invariant mass for the inclusive and signal fiducial regions with $\mjj > 1.0$~\TeV.  Both statistical
(inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios of the theoretical 
predictions to the data (the bottom panel in each distribution). }
\label{unfolding:EWKcombined_measurementdijetmass1Dhighmass10}
\end{figure}

\begin{figure}[tbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dy12_1D_highmass10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dy12_1D_signal10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dy12_1D_highmass15}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dy12_1D_highmass20}
\caption{Unfolded normalized differential EW~\wjets production cross sections as a function of 
$\dyjj$ for the inclusive fiducial region with three thresholds on the dijet invariant mass, 1.0~\TeV~(top left), 
1.5~\TeV~(bottom left), and 2.0~\TeV~(bottom right), and for the signal-enriched fiducial region with a minimum 
dijet invariant mass of 1.0~\TeV~(top right).  Both statistical (inner bar) and total (outer bar) measurement 
uncertainties are shown, as well as ratios of the theoretical predictions to the data (the bottom panel in each 
distribution). }
\label{unfolding:EWKcombined_measurementdy121Dhighmass10}
\end{figure}

\begin{figure}[tbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dphi12_1D_highmass10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_dphi12_1D_signal10}
\caption{Unfolded normalized differential EW~\wjets production cross sections as a function 
of the azimuthal angle between the two leading jets, for the inclusive and signal fiducial regions with 
$\mjj > 1.0$~\TeV.  Both statistical (inner bar) and total (outer bar) measurement uncertainties are shown, 
as well as ratios of the theoretical predictions to the data (the bottom panel in each distribution).}
\label{unfolding:EWKcombined_measurementdphi1Dhighmass10}
\end{figure}

\begin{figure}[tbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_j1pt_1D_highmass10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_j1pt_1D_signal10}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_j1pt_1D_highmass15}
\includegraphics[width=0.48\textwidth]{figures/unfolding/normalisedXsec/EWKmeasurement_combined_j1pt_1D_highmass20}
\caption{Unfolded normalized differential EW~\wjets production cross sections as a function of the 
leading-jet $\pt$ for the inclusive fiducial region with three thresholds on the dijet invariant mass (1.0~\TeV, 
1.5~\TeV, and 2.0~\TeV), and for the signal-enriched fiducial region with a minimum dijet invariant mass of 
1.0~\TeV.  Both statistical (inner bar) and total (outer bar) measurement uncertainties are shown, as well as ratios 
of the theoretical predictions to the data (the bottom panel in each distribution). }
\label{unfolding:EWKcombined_measurementj1pt1Dhighmass10}
\end{figure}

Figure~\ref{unfolding:EWKcombined_measurementngapjets1Dhighmass10_15} shows the normalized cross sections as a 
function of the number of jets with $\pt>30$~\GeV~emitted into the rapidity interval bounded by the two leading jets, 
for two dijet invariant-mass thresholds ($1.0$~\TeV~and $2.0$~\TeV) in the inclusive fiducial region.  The 
measured fraction of EW \wjets events with no additional central jets is higher than that of QCD+EW \wjets events 
(which are shown in Figure~\ref{unfolding:norm_measurementngapjets}).  The impact of QCD--EW interference on this 
observable is negligible. 

Figure~\ref{unfolding:EWKcombined_measurementdijetmass1Dhighmass10} shows the normalized cross section as a function 
of dijet invariant mass for the inclusive and signal regions with $\mjj>1.0$~\TeV.  This observable is used to 
extract the EW~\wjets signal in Section~\ref{sec:xsec} and is well described by the Monte Carlo simulation within 
uncertainties.  Figure~\ref{unfolding:EWKcombined_measurementdy121Dhighmass10} shows the distribution of the rapidity 
interval between the two leading jets in the inclusive and signal regions with $\mjj>1.0$~\TeV, and for the inclusive 
region with invariant-mass thresholds of 1.5 and 2.0~\TeV.  Significant interference contributions are observed at low 
$\dyjj$, where modelling uncertainties associated with the strong \wjets subtraction also limit the precision.

Figure~\ref{unfolding:EWKcombined_measurementdphi1Dhighmass10} shows the normalized cross section as a function of the 
azimuthal angle between the two leading jets for the inclusive and signal fiducial regions with $\mjj>1.0$~\TeV.  
This observable is sensitive to the presence of anomalous CP-violating couplings~\cite{vbfcp}. 

All measured distributions in 
Figures~\ref{unfolding:EWKcombined_measurementngapjets1Dhighmass10_15}--\ref{unfolding:EWKcombined_measurementdphi1Dhighmass10} 
are modelled well by both \powheg + \pythia and \sherpa.
Figure~\ref{unfolding:EWKcombined_measurementj1pt1Dhighmass10} shows the distribution of the normalized cross section 
as a function of leading-jet $\pt$ in the inclusive fiducial region with $\mjj > 1.0$~\TeV, 1.5~\TeV, and 2.0~\TeV, 
and the electroweak signal region with $\mjj > 1.0$~\TeV.  Good agreement with the predictions is seen at low dijet 
invariant mass; at higher masses ($\mjj>1.5$~\TeV) both the \powheg + \pythia and \sherpa predictions give a harder 
spectrum than observed in the data.  This feature is not seen for \powheg + \pythia in the QCD+EW \wjets production 
cross sections shown in Figure~\ref{unfolding:combined_measurementj1pt1DantiLC}.  The overestimation of rates at 
high jet \pt may be reduced by the inclusion of NLO electroweak corrections\,\cite{openloops1}.


\subsection{Integrated fiducial cross sections}
\label{sec:intxsec}

Integrated cross sections for \wjets production are determined in each fiducial region.
Figure~\ref{unfolding:intxsec_public} and Table~\ref{unfolding:intxsec_public_table} show the measured integrated 
production cross sections times branching fractions ($\sigma^\mathrm{fid}_{Wjj}\times {\cal{B}}_{W\rightarrow \ell \nu}$) 
for QCD+EW \wjets production and, in high dijet invariant-mass regions, for EW \wjets production. 
Also shown is the value of the EW \wjets cross section extracted from the constrained fit described in 
Section~\ref{sec:fidxsresults}.  All measurements are compared to predictions from \powheg + \pythia.

\begin{table*}[!htbp]
\caption{
Integrated production cross sections times branching fractions for QCD+EW \wjets production and EW \wjets 
production in each measured particle-level fiducial region and the equivalent prediction from \powheg + \pythia.
The uncertainties displayed are the values of the statistical and systematic uncertainties added in quadrature.}
\label{unfolding:intxsec_public_table}
\begin{center}
\begin{tabular}{lcccc}
\toprule
Fiducial region & \multicolumn{4}{c}{$\sigma^\mathrm{fid}_{Wjj} \times {\cal{B}}_{W\rightarrow \ell \nu}$ [fb]} \\
                & \multicolumn{2}{c}{QCD+EW} & \multicolumn{2}{c}{EW} \\
                & Data & \powheg + \pythia & Data & \powheg + \pythia \\
\midrule
Inclusive $\mjj>0.5$~\TeV & $1700\pm 110$ & $1420\pm 150$ & --- & --- \\[0.1ex]
Inclusive $\mjj>1.0$~\TeV & $263\pm 21$ & $234\pm 26$ & $64\pm 36$ & $52\pm 1$\\[0.1ex]
Inclusive $\mjj>1.5$~\TeV & $56\pm 5$ & $53\pm 5$ & $20\pm 8$ & $19\pm 0.5$ \\[0.1ex]
Inclusive $\mjj>2.0$~\TeV & $13\pm 2$ & $14\pm 1$ & $5.6\pm 2.1$ & $6.9\pm 0.2$\\[0.1ex]
Forward-lepton & $545\pm 39$ & $455\pm 51$ & --- & ---\\[0.1ex]
Central-jet & $292\pm 36$ & $235\pm 28$ & --- & ---\\[0.1ex]
Forward-lepton/central-jet & $313\pm 30$ & $265\pm 32$ & --- & ---\\[0.1ex]
Signal $\mjj>0.5$~\TeV & $546\pm 35$ & $465\pm 39$ & $159\pm 25$ & $198\pm 12$\\[0.1ex]
Signal $\mjj>1.0$~\TeV & $96\pm 8$ & $89\pm 7$ & $43\pm 11$ & $41\pm 1$\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{figures/unfolding/intXsec/intXsecSummary_combined.pdf}
\caption{Integrated production cross sections times branching fractions for QCD+EW \wjets production 
(solid data points) and EW \wjets production (open data points) in each measured particle-level fiducial 
region in a single lepton channel; EW \wjets production is only measured in a subset of fiducial regions 
where there is sufficient purity.  For each measurement the error bar represents the statistical and 
systematic uncertainties summed in quadrature.  Comparisons are made to predictions from \powheg + \pythia 
for QCD+EW or EW~\wjets production.  The bottom pane shows the ratio of data to \powheg + \pythia predictions.}
\label{unfolding:intxsec_public}
\end{figure}

The measured data and \powheg + \pythia predictions are broadly compatible across all measured fiducial volumes. 
In fiducial regions dominated by strong \wjets production, the measured cross sections are approximately 15--20\% 
higher than predictions.  The harder \mjj distribution in \powheg + \pythia relative to data 
(Figures~\ref{unfolding:combined_measurementdijetmass1Dinclusive} and~\ref{unfolding:combined_measurementdijetmass1Dsignal})
results in a progressively decreasing ratio of measured to predicted cross sections for combined 
QCD+EW~\wjets production.  The measured EW \wjets production 
cross sections have larger uncertainties than the precisely constrained fiducial electroweak \wjets cross-section 
measurement described in Section~\ref{sec:fidxsresults} (also shown in Figure~\ref{unfolding:intxsec_public}).

The measurements of electroweak $\wjets$ fiducial cross sections are compared to measurements of electroweak 
$Zjj$ production and VBF Higgs boson production in Figure~\ref{fig:LHCEWKHiggsxsec}.  These other measurements 
are extrapolated to lower dijet mass (for $Zjj$ production) or to inclusive production (for Higgs boson 
production) so their apparent cross sections are increased relative to the \wjets fiducial cross sections.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.97\textwidth]{figures/EWK_xsec_Summary_withHiggs.pdf}
\caption{Measurements of the cross sections times branching fractions of electroweak production of a single 
$W$, $Z$, or Higgs boson with two jets at high dijet invariant mass and in fiducial measurement regions.  For 
each measurement the error bar represents the statistical and systematic uncertainties summed in quadrature.  
Shaded bands represent the theory predictions.  The \mjj threshold defining the fiducial $Zjj$ region differs 
between ATLAS and CMS, leading to different inclusive cross sections. }
\label{fig:LHCEWKHiggsxsec}
\end{figure}

